Analyzing Behavioural Scenarios over Tabular Specifications Using Model Checking

Tabular notations, in particular SCR specifications, have proved to be a useful means for formally describing complex requirements. The SCR method offers a powerful family of analysis tools, known as the SCR Toolset, but its availability is restricted by the Naval Research Laboratory of the USA. This toolset applies different kinds of analysis considering the whole set of behaviours associated with a requirements specification. In this paper we present a tool for describing and analyzing SCR requirements descriptions, that complements the SCR Toolset in two aspects. First, its use is not limited by any institution, and resorts to a standard model checking tool for analysis; and second, it allows to concentrate the analysis to particular sets of behaviours (subsets of the whole specifications), that correspond to particular scenarios explicitly mentioned in the specification. We take an operational notation that allows the engineer to describe behavioural "scenarios" by means of programs, and provide a translation into Promela to perform the analysis via Spin, an efficient off-the-shelf model checker freely available. In addition, we apply the SCR method to a Pacemaker system and we use its tabular specification as a running example of this article.

==> eptcsdata.tex <==
\providecommand{\firstpage}{71}
\providecommand{\publicationstatus}{Nazareno Aguirre, Leila Ribeiro (Eds.):\\
First Latin American Workshop on Formal Methods (LAFM 2013)\\
EPTCS 139, 2014, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.139.8}{10.4204/EPTCS.139.8}}
\pdfoutput=1

